Continuous Verification of Large Embedded Software using SMT-Based Bounded Model Checking

The complexity of software in embedded systems has increased significantly over the last years so that software verification now plays an important role in ensuring the overall product quality. In this context, SAT-based bounded model checking has been successfully applied to discover subtle errors, but for larger applications, it often suffers from the state space explosion problem. This paper describes a new approach called continuous verification to detect design errors as quickly as possible by looking at the Software Configuration Management (SCM) system and by combining dynamic and static verification to reduce the state space to be explored. We also give a set of encodings that provide accurate support for program verification and use different background theories in order to improve scalability and precision in a completely automatic way. A case study from the telecommunications domain shows that the proposed approach improves the error-detection capability and reduces the overall verification time by up to 50%.

==> 01-introduction.tex <==
%------------------------------------------------------
\section{Introduction}
\label{01-introduction}
%------------------------------------------------------

Embedded computer systems are used in a wide range of sophisticated
applications, such as mobile phones or set-top boxes providing internet
connectivity. The functionality demanded for such systems has increased
significantly and an increasing number of functions are implemented in
software rather than hardware. As a consequence, the verification of the
software design and the correctness of its implementation have become
increasingly difficult. 

Bounded model checking (BMC) has been successfully applied to verify
embedded software and discovered subtle errors in real
designs~\cite{handbook09}. 
BMC generates verification conditions (VCs) that
reflect the exact path in which a statement is executed,
the context in which a given function is called, and the bit-accurate
representation of the expressions. Proving the validity of these VCs
remains the main performance bottleneck in verifying large embedded
software, despite attempts to cope with increasing system complexity by
applying SMT (Satisfiability Modulo Theories)
solvers~\cite{Armando09,Cordeiro09,Ganai06}. 

We address this bottleneck with a new concept called \emph{continuous
verification}. It aims to automatically detect design errors and
integration problems as quickly as possible by exploiting information from
the software configuration management (SCM) system, systematically focusing the
verification effort on new or modified functions. We use equivalence
checking to determine whether modified functions need to be re-verified
formally and we use existing test cases to reduce the search space for
the model checker, thus combining dynamic and static verification. We show
that the continuous verification approach substantially reduces the
verification time of large embedded software. 

We also exploit the different background theories of SMT solvers and
combine different theories and solvers, based on an analysis of the
syntactic structure of a given ANSI-C program.  We then demonstrate that
this combination significantly improves the performance of software model
checking for a wide range of embedded software benchmarks from the 
telecommunications domain.  
%%% To the best of our knowledge, 
This is the first work that exploits
the syntactic structure of an ANSI-C program in order to combine different
encodings and SMT solvers for BMC of embedded software. 
%%% before checking the VCs emerging from the BMC
%%% instances of embedded software. 

We describe how these new (compared to our previous work~\cite{Cordeiro09})
contributions are realized in ESBMC, the Efficient SMT-Based Bounded Model
Checker. ESBMC extends CBMC~\cite{Clarke04} to support different theories
and different SMT solvers and to make use of high-level information to
simplify and reduce the unrolled formula size. Experimental results show
that our approach scales significantly better than both the SAT-based and
SMT-based versions of the CBMC model checker. In addition, the continuous
verification approach and the combination of different encodings and
solvers allow us to go deeper into the system (compared to software model
checkers only) and explore more exhaustively the state space (compared to
testing only). This hybrid solution is suitable for checking properties in
large state spaces.


==> 05-related-work.tex <==
%------------------------------------------------------
\section{Related Work}
\label{06-related-work}
%------------------------------------------------------

One way of tackling large verification problems is to leverage both
parallelism and search diversity~\cite{HolzmannJG08}. Holzmann et al.\ describe the 
Swarm tool that allows to use different search strategies on
multi-core machines~\cite{HolzmannJG08}. It is the main interface to the
SPIN model checker to verify larger systems. This approach, however,
involves large communication overhead and does not take into account
information from the SCM system in order to focus the verification effort
on new and/or modified functions. 

\comment{
In another related work, Holzmann et al. explore the availability of large chunks of memory to go deeper into the state space exploration. However, the authors do not consider that the search modes implemented in the SPIN model checker (mainly based on depth-first search) still remain the main performance bottleneck to verify larger system~\cite{HolzmannB07}.}

Peled proposes a set of combinations between model checking and testing, which includes black box checking, adaptive model checking, and unit checking~\cite{Peled03}. However, he does not consider the development history from the SCM system and also uses explicit model checking based on automata theory, which does not scale well due to the number of program variables and data type widths~\cite{DSilvaKW08}. In addition, Peled only describes the techniques, but does not apply it to any
commercial product. Gunter and Peled~\cite{GunterP05} extend this approach by proposing a symbolic verification approach for a unit of code, also called unit checking.  The authors, however, apply this approach only to check whether a complex number diverges to infinity, while we focus on the verification of large embedded software. Sen proposes an approach to execute a program concretely and symbolically by combining random testing and symbolic execution~\cite{Sen07}. This approach, however, might fail to compute concrete values that satisfy a given path constraint due to the constraint solver performance.

SMT-based BMC is gaining popularity in the formal verification community
due to the advent of sophisticated SMT solvers built over efficient SAT
solvers~\cite{Boolector09,Z08}. Ganai and Gupta describe a verification
framework for BMC which extracts high-level design information from an
extended finite state machine (EFSM) and applies several techniques to
simplify the BMC problem~\cite{Ganai06}. However, the authors flatten the 
structures and arrays into scalar variables in such a way that they use only 
the theory of integer and real arithmetic, which does not reflect precisely the ANSI-C semantics. 
Armando et al.\ also propose a BMC approach using SMT solvers for ANSI-C
programs~\cite{Armando09}. In this approach, however, they only make use of
linear arithmetic (addition and multiplication by constants), arrays,
records and bit-vectors and as a consequence, their SMT-CBMC prototype does
not address important constructs of the ANSI-C language (e.g., non-linear
arithmetic and bit-shift operations). 

Recently, a number of static checkers have been developed in order to trade
off scalability and precision. Calysto is a static checker that is able to
verify VCs related to arithmetic overflow, nil-pointer dereferencing and
assertions specified by the user~\cite{bh08calysto}. The VCs are passed to
the SMT solver SPEAR which supports bit-vector arithmetic and is customized
for the VCs generated by Calysto. However, Calysto does not support
float-point operations and unsoundly approximates loops by unrolling them
only once. As a consequence, soundness is relinquished for performance.
Saturn is another efficient static checker that scales to larger systems,
but with the drawback of losing precision by supporting only the most
common integer operators and performing at most two unwindings of each
loop~\cite{saturn05}.


==> 06-conclusion.tex <==
%------------------------------------------------------
\section{Conclusions}
\label{07-conclusion}
%------------------------------------------------------

In this work, we have defined a new concept called \emph{continuous verification} and we have applied it to the verification of large embedded software used in the telecommunications domain. In addition, we have described a new set of encodings that allow us to reason accurately about embedded software by discovering subtle bugs in several industrial applications and to scale for large embedded software. Furthermore, the experimental results show that our SMT-based model checker (ESBMC) outperforms both the SAT-based and SMT-based CBMC~\cite{Clarke04} model checker if we consider the verification of embedded software. As a result, our approach represents a promising direction to improve the state space coverage and to verify quickly the negation of properties in larger state spaces.

\comment{
For future work, we intend to investigate the verification of concurrent software and the application of termination analysis.}

